A JWST Study of Stardust. I. Infrared Spectroscopy of Comet 81P/Wild 2 and Overall Composition

We report observations of comet 81P/Wild 2, target of the Stardust sample return mission, on UT 2023 March 20 and 24 at a heliocentric distance ($r_H$) of 1.85 au using the NIRSpec and MIRI integral field unit spectrographs on board the James Webb Space Telescope (JWST). This study is the first compositional comparison between JWST remote-sensing spectroscopy of a solar system object against terrestrial analysis of its returned samples. We securely detected molecular emission from H$_2$O, CH$_4$, C$_2$H$_6$, CH$_3$OH, CO, CO$_2$, $^{13}$CO$_2$, OCS, HCN, and CN and find molecular abundances consistent within $2\sigma$ with those reported during previous perihelion passages. The water ortho-to-para ratio was $2.76\pm0.05$, and the $^{12}$CO$_2$/$^{13}$CO$_2$ ratio was $85\pm4$. Thermal emission from the nucleus and dust was detected and modeled, providing an effective nucleus radius of $1.77\pm0.04$ km and a dust composition (relative mass fraction of the submicron grains) of $\sim36\%$ amorphous carbon, $\sim25\%$ amorphous Mg:Fe olivine, $\sim23\%$ Mg-rich crystalline olivine, and $\sim15\%$ amorphous Mg:Fe pyroxene. The crystalline mass fraction of the sub-micron grains in the coma was $0.362\pm0.003$. Comparison of the JWST-derived thermal model against the fine-grained materials in Stardust returned samples demonstrates complementarity between the missions, with each most sensitive to a different population of the coma dust grains.

==> Modeling.tex <==
\section{Discussion and Interpretation}\label{sec:discussion}
Our results show that...

\subsection{Comparison to Previous Observations}\label{subsec:previous}
Our results are consistent with previous observations...

\subsection{Connection to Primitive Environments}\label{subsec:primitive}

PAHs are found in diverse environments, from evolved stars, to the ISM, to meteorites, to some (but not all) interplanetary dust particles (IDPs) and cometary samples \cite{Li2020}. First proposed to account for the ``unidentified infrared bands'' (UIR), PAHs are identified by their near- and mid-infrared bands. Rather than identifying an individual PAH molecule (e.g., naphthalene), these bands are diagnostic of the complex mixture of PAHs in an environment, with the band ratios indicative of the average PAH size \citep[i.e., 3.3 $\mu$m/11.3 $\mu$m ratio][]{Croiset2016} and average PAH charge \citep[7.7 $\mu$m/11.3 $\mu$m][]{Galliano2008}. 

Individual bands provide further information, with the presence of the 6.2 $\mu$m band indicative of significant nitrogen-substituted PAHs (PANHs) and the 11.3 $\mu$m band attributed to large neutral PAHs \citep{Cami2011,Peeters2002}. The wavelength of the 7.7 $\mu$m band peak is correlated with the effective temperature of the circumstellar environment in which the PAHs formed \citep{Sloan2007}, while offsets in the peak wavelength of other features have been attributed to N- or O-substitution \citep{Evans2005,Ootsubo2020}. Combined with a taxonomic classification system for PAH sources based on the relative intensities and positions of each band \citep{Peeters2002}, this suggests that PAH spectra in a given object are indicative of the radiation processing that they have been exposed to, from little processing (Class C objects, e.g., evolved stars) to moderate processing (Class B, e.g. Herbig Ae/Be stars) to extensive processing (Class A, e.g., the ISM). Thus, measuring (or stringently constraining) the PAH content of comets can provide insights into the processing experienced by the material incorporated into their nuclei.

Just as cometary enrichment in D and $^{15}$N in coma volatiles provide evidence for the incorporation of primitive material into their nuclei \cite{Bockelee-Morvan2015}, the nature of the PAHs in comets may provide a window to test the heritage of cometary soluble refractory organics. A survey of comets found an unidentified feature at 3.28 $\mu$m in  near-IR spectra, but would have required an excessively high  abundance to reproduce its intensity \citep{Bockelee1995}. \textit{Vega 2} spectra of 1P/Halley from 340 -- 390 nm were consistent with phenanthrene and naphthalene \citep{Clairemidi2004,Moreels1994}. \textit{Rosetta} ROSINA detected the small PAH naphthalene at small quantities in the coma of 67P \citep{Altwegg2019}. \textit{Spitzer} mid-IR studies reported PAH features in the \textit{Deep Impact} ejecta of 9P/Tempel 1 (although not in the pre-impact coma) \citep{Lisse2006} but without modeling of the overlying water vapor. An upper limit in C/2003 K4 was based on residual flux at the position of the 6.2 $\mu$m feature \citep{Woodward2007}. 

Further detections were claimed in archival \textit{ISO} spectra of  C/1995 O1 (Hale-Bopp) \citep{Lisse2007}, yet these were controversial \citep{Crovisier2008}. More recently, UIR features were found in comet 21P and attributed to N- or O-bearing PAHs \citep{Ootsubo2020}. In both the 9P/Tempel 1 ejecta and 21P/Giacobini-Zinner, band ratios of the PAH features were more consistent with ionized PAHs than with neutrals, possibly consistent with PAH ionization occurring in ice-phase grain-surface chemistry before incorporation into the nucleus because the UV solar radiation field supports neutral PAHs. 

More recent results from space-based assets have brought the PAH content of comets into clearer view, with detailed analyses from the \textit{Rosetta} mission to comet 67P/Churyumov-Gerasimenko and JWST observations of comet C/2017 K2 (PanSTARRS) suggesting their composition reflects a presolar history and a long sequence of material processing beginning in the interstellar medium \citep[ISM;][]{Hanni2022,Woodward2025}. 

Our analysis of PAH emission shows...

\subsection{Connection to the Stardust Return Samples}\label{subsec:stardust}
Our results are complementary to the Stardust analysis...
